Extrapolatable Relational Reasoning With Comparators in Low-Dimensional Manifolds

While modern deep neural architectures generalise well when test data is sampled from the same distribution as training data, they fail badly for cases when the test data distribution differs from the training distribution even along a few dimensions. This lack of out-of-distribution generalisation is increasingly manifested when the tasks become more abstract and complex, such as in relational reasoning. In this paper we propose a neuroscience-inspired inductive-biased module that can be readily amalgamated with current neural network architectures to improve out-of-distribution (o.o.d) generalisation performance on relational reasoning tasks. This module learns to project high-dimensional object representations to low-dimensional manifolds for more efficient and generalisable relational comparisons. We show that neural nets with this inductive bias achieve considerably better o.o.d generalisation performance for a range of relational reasoning tasks. We finally analyse the proposed inductive bias module to understand the importance of lower dimension projection, and propose an augmentation to the algorithmic alignment theory to better measure algorithmic alignment with generalisation.

==> sections/impact.tex <==
\section*{Broader Impact}
The generalisation capability of AI systems is a key factor affecting its applicability in industrial and daily scenarios. The system's lack of generalisation to unseen situations will lead to safety, security and financial risks. Examples includes autonomous driving vehicles not recognising unseen objects and crashing into them because this object has not been included in the training data. Our work aim to improve NN's generalisation ability for relational reasoning tasks, which are performed in many broader tasks such as autonomous driving and industrial component assembly. While our work is exploratory as we focus on abstract visual reasoning tasks, we believe future extensions of our work will help making applications of AI systems safer and more viable. 

==> sections/pruning_not_included.tex <==
\subsection{Pruning}

\begin{figure}[h!]
\centering

\begin{subfigure}{.325\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/Heatmap_plot_baseline_v2_few_orig_eq.jpg}
  \caption{baseline}
  \label{fig:baseline}
\end{subfigure}
\begin{subfigure}{.325\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/Heatmap_plot_baseline_v2_few_eq.jpg}
  \caption{baseline pruned}
  \label{fig:baseline_pruned}
\end{subfigure}
\begin{subfigure}{.325\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/Heatmap_plot_dsprites_comparator_v2_few_eq.jpg}
  \caption{baseline pruned}
  \label{fig:1d_comp}
\end{subfigure}
\caption{Plots of the learnt ``equal'' function values over ground truth vertical position values of compared objects. Blue squares indicate values within the training range. Figure (a) shows the function learnt by baseline. (b) shows the function of the pruned and re-trained baseline. (c) shows the function of 1-d comparator.}
\label{fig:2d_space}
\end{figure}
